Centralized Matching with Incomplete Information

We study the impacts of incomplete information on centralized one-to-one matching markets. We focus on the commonly used Deferred Acceptance mechanism (Gale and Shapley, 1962). We show that many complete-information results are fragile to a small infusion of uncertainty about others' preferences.

==> examples/ex_quantile_fragility.tex <==
\begin{center}
\begin{tikzpicture}
\matrix (m)[matrix of nodes, style={nodes={color = white, rectangle,draw,minimum width=3em, line width=0pt}}, minimum height=2em, row sep=-\pgflinewidth, column sep=-\pgflinewidth]
{
$\lambda$	\\ 
\color{black}$\lambda$		\\ 
$\lambda$	\\
};
\begin{pgfonlayer}{myback}
\fillpattern[north east lines][orange]{m-2-1}{m-2-1}
\end{pgfonlayer}
\end{tikzpicture}
\quad
\begin{tikzpicture}
\matrix (m)[matrix of nodes, style={nodes={rectangle,draw,minimum width=4em}}, minimum height=2em, row sep=-\pgflinewidth, column sep=-\pgflinewidth]
{
{{\color{white}/}$\bm{3,2}${\color{white}/}} & $1,5$ & {\color{white}/}$2,2${\color{white}/}\\
    $2,5$ & {{\color{white}/}$\bm{3,2}${\color{white}/}} & $1,5$\\
    {\color{white}/}$3,1${\color{white}/} & {\color{white}/}$1,1${\color{white}/} & {\color{white}/}$\bm{2,1}${\color{white}/}	\\
};

\begin{pgfonlayer}{myback}
\node at (0,1.6) {$U(1)$};
\fillpattern[north east lines][orange]{m-2-1}{m-2-1}
\fillpattern[north east lines][orange]{m-1-3}{m-1-3}
\fillpattern[north east lines][orange]{m-3-2}{m-3-2}
\end{pgfonlayer}
\end{tikzpicture}
\quad
\begin{tikzpicture}
\matrix (m)[matrix of nodes, style={nodes={rectangle,draw,minimum width=4em}}, minimum height=2em, row sep=-\pgflinewidth, column sep=-\pgflinewidth]
{
{{\color{white}/}$\bm{3,2}${\color{white}/}} & $1,5$ & {\color{white}/}$2,2${\color{white}/}\\
    $1,5$ & {{\color{white}/}$\bm{3,2}${\color{white}/}} & $2,5$\\
    {\color{white}/}$1,1${\color{white}/} & {\color{white}/}$2,1${\color{white}/} & {\color{white}/}$\bm{3,1}${\color{white}/}	\\
};

\begin{pgfonlayer}{myback}
\node at (0,1.6) {$U(2)$};
\fillpattern[north east lines][orange]{m-1-2}{m-1-2}
\fillpattern[north east lines][orange]{m-2-3}{m-2-3}
\end{pgfonlayer}
\end{tikzpicture}
\end{center}

